Improving Branch Prediction By Modeling Global History with Convolutional Neural Networks

CPU branch prediction has hit a wall--existing techniques achieve near-perfect accuracy on 99% of static branches, and yet the mispredictions that remain hide major performance gains. In a companion report, we show that a primary source of mispredictions is a handful of systematically hard-to-predict branches (H2Ps), e.g. just 10 static instructions per SimPoint phase in SPECint 2017. The lost opportunity posed by these mispredictions is significant to the CPU: 14.0% in instructions-per-cycle (IPC) on Intel SkyLake and 37.4% IPC when the pipeline is scaled four-fold, on par with gains from process technology. However, up to 80% of this upside is unreachable by the best known branch predictors, even when afforded exponentially more resources. New approaches are needed, and machine learning (ML) provides a palette of powerful predictors. A growing body of work has shown that ML models are deployable within the microarchitecture to optimize hardware at runtime, and are one way to customize CPUs post-silicon by training to customer applications. We develop this scenario for branch prediction using convolutional neural networks (CNNs) to boost accuracy for H2Ps. Step-by-step, we (1) map CNNs to the global history data used by existing branch predictors; (2) show how CNNs improve H2P prediction in SPEC 2017; (3) adapt 2-bit CNN inference to the constraints of current branch prediction units; and (4) establish that CNN helper predictors are reusable across application executions on different inputs, enabling us to amortize offline training and deploy ML pattern matching to improve IPC.

==> spec_stats_table.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t!]
  \centering
  \scriptsize
  \begin{tabularx}{\textwidth}{l|r|*{4}{r|}r|*{4}{r|}r|r}%%||r|r|r|r|r||r|r}
    \hline
    \hline
    \multirow{3}{*}{\parbox{1.825cm}{\centering SPECint2017 Benchmark}} &
    \multirow{3}{*}{\parbox{0.75cm}{\centering Avg \# Phases}} &
    \multicolumn{4}{c|}{\# Static Branches} &
    \multirow{3}{*}{\parbox{0.8cm}{\centering \# App. Inputs}} &
    \multicolumn{2}{c|}{\parbox{2cm}{\centering H2P Appearance Across Inputs}} &
    \multicolumn{2}{c|}{\parbox{1.5cm}{\centering \# Static H2P Branches}} &
    \multirow{3}{*}{\parbox{1.6cm}{\centering Avg. Dyn. Execs per H2P
        per Region}} &
    \multirow{3}{*}{\parbox{1.25cm}{\centering \% Mispreds due to
        H2Ps per Region}}\\
    \cline{3-6}\cline{8-11}
    &
    &
    \multirow{2}{*}{\parbox{0.75cm}{\centering Total}} &
    \multirow{2}{*}{\parbox{0.80cm}{\centering Med per Reg.}} &
    \multirow{2}{*}{\parbox{0.80cm}{\centering Min per Reg.}} &
    \multirow{2}{*}{\parbox{0.80cm}{\centering Max per Reg.}} &
    & 
    \multirow{2}{*}{\parbox{0.80cm}{\centering Total}} &
    \multirow{2}{*}{\parbox{0.8cm}{\centering 3+ Inputs}} &
    \multirow{2}{*}{\parbox{0.80cm}{\centering Avg per Input}} &
    \multirow{2}{*}{\parbox{0.80cm}{\centering Avg per Reg.}} & &
    \\
    & & & & & & & & & & & & \\
    & & & & & & & & & & & & \\
    \hline\hline
    600.perlbench\_s & 6.5 & 13,865 & 1,863 & 435 & 11,276 & 4 & 62 & 16 & 21.5 & 1 & 93,815 & 17.3\% \\
    602.gcc\_s$\dagger$ & 13.2 &  54,605  &  6,411  &  830  &  29,043  & 13 & 806 & 326 & 200 & 6 &  44,046  & 13.5\% \\
    605.mcf\_s & 11.4 &  1,755  &  99  &  93  &  1,536  & 8 & 29 & 20 & 19 & 10 &  249,195  & 96.9\% \\
    620.omnetpp\_s & 11.8 &  7,099  &  823  &  306  &  4,344  & 5 & 46 & 28 & 28 & 8 &  74,630  & 77.6\% \\
    623.xalancbmk\_s & 7.5 &  8,563  &  3,103  &  1,431  &  5,753  & 4 & 28 & 8 & 14.5 & 6 &  75,329  & 28.6\% \\
    625.x264\_s & 13.9 &  4,892  &  1,068  &  138  &  2,181  & 14 & 23 & 7 & 6 & 1 &  65,593  & 54.2\% \\
    631.deepsjeng\_s & 9.4 &  3,162  &  856  &  1  &  1,754  & 12 & 68 & 49 & 40 & 13 &  44,412  & 31.2\% \\
    641.leela\_s & 8.8 &  3,623  &  582  &  11  &  1,599  & 10 & 77 & 68 & 56.5 & 34 &  35,614  & 66.4\% \\
    648.exchange2\_s & 8.4 &  3,765  &  1,330  &  611  &  3,326  & 5 & 38 & 19 & 20 & 7 &  142,320  & 44.7\% \\
    657.xz\_s & 7.6 &  2,373  &  211  &  89  &  1,794  & 5 & 163 & 50 & 63 & 10 &  75,759  & 80.5\% \\
    \hline
    MEAN & 9.5 & 5,455  & 1,104  & 346  & 3,729  & 7 & 59 & 29 & 30 & 10 &  95,185  & 55.3\% \\
    \hline\hline
      %% & & & \\% & & & & & & \\
  \end{tabularx}
  \caption{Summary statistics of our SPECint 2017 data set, which
    includes an expanded collection of inputs for each benchmark.  The various
    metrics shown are averaged over 10B-instruction traces from each
    input. $\dagger$\texttt{gcc} is an outlier benchmark because its
    code footprint is many times larger than the others, leading to
    different behaviors under TAGE-SC-L. We hold it out from the mean
    statistic and mark it for future study.  }
  \label{tab:spec2017}
 \end{table*}

